Structural Parameters for Steiner Orientation

We consider the \textsc{Steiner Orientation} problem, where we are given as input a mixed graph $G=(V,E,A)$ and a set of $k$ demand pairs $(s_i,t_i)$, $i\in[k]$. The goal is to orient the undirected edges of $G$ in a way that the resulting directed graph has a directed path from $s_i$ to $t_i$ for all $i\in[k]$. We adopt the point of view of structural parameterized complexity and investigate the complexity of \textsc{Steiner Orientation} for standard measures, such as treewidth. Our results indicate that \textsc{Steiner Orientation} is a surprisingly hard problem from this point of view. In particular, our main contributions are the following: (1) We show that \textsc{Steiner Orientation} is NP-complete on instances where the underlying graph has feedback vertex number 2, treewidth 2, pathwidth 3, and vertex integrity 6; (2) We present an XP algorithm parameterized by vertex cover number $\mathrm{vc}$ of complexity $n^{\mathcal{O}(\mathrm{vc}^2)}$. Furthermore, we show that this running time is essentially optimal by proving that a running time of $n^{o(\mathrm{vc}^2)}$ would refute the ETH; (3) We consider parameterizations by the number of undirected or directed edges ($|E|$ or $|A|$) and we observe that the trivial $2^{|E|}n^{\mathcal{O}(1)}$-time algorithm for the former parameter is optimal under the SETH. Complementing this, we show that the problem admits a $2^{\mathcal{O}(|A|)}n^{\mathcal{O}(1)}$-time algorithm. In addition to the above, we consider the complexity of \textsc{Steiner Orientation} parameterized by $\mathrm{tw}+k$ (FPT), distance to clique (FPT), and $\mathrm{vc}+k$ (FPT with a polynomial kernel).

==> Figures/parameter.tex <==

\begin{figure}[ht]
\centering
\scalebox{0.8}{ % Start scaling
\begin{tikzpicture}[
  every node/.style={draw, rectangle, rounded corners, align=center, minimum width=2.8cm, font=\small},
  paraNP/.style={text=red!80!black,draw, rectangle,  double, sharp corners},
  XP/.style={text=blue, draw, rectangle, sharp corners},
  FPTAS/.style={text=orange,dash pattern=on 3pt off 2pt},
  FPT/.style={text=green!30!black,thick},
  Open/.style={text=black,dash pattern=on 3pt off 2pt,sharp corners,thick},
%  ->, >=Stealth
]

% Nodes positioned to match the original image
% \node[paraNP] (diameter) at (-6.5,4) {diameter};
% \node[paraNP] (dn) at (-6.5,2) {domination number~\cite{tcs/Tale25}};
\node[Open] (ccn) at (-6.5,-0.5) {clique cover$^*$};
\node[Open] (cvd) at (-4,1) {cluster vertex deletion$^*$};
\node[FPT] (dtc) at (-6.5,-3.5) {distance to clique$^*$};


%\node[XP] (nd) at (-4,0.5) {neighborhood diversity};


\node[paraNP] (cw) at (-0.5,4) {cliquewidth};
\node[paraNP] (tw) at (-0.5,2.5) {treewidth};
\node[paraNP] (pw) at (-0.5,1) {pathwidth};
\node[paraNP] (td) at (-0.5,-0.5) {tree-depth$^*$};
\node[FPT] (vi) at (-0.5,-2) {vertex integrity$^*$};
\node[FPT] (vc) at (-0.5,-3.5) {vertex cover~\cite{tcs/FominFG24}};


\node[paraNP] (fvs) at (3.5,1) {feedback vertex set};
\node[paraNP] (dtp) at (3.5,-0.5) {distance to path forest$^*$ \cite{tcs/Tale25}};
\node[FPT] (fes) at (7,-2) {feedback edge set~\cite{tcs/FominFG24}};


%\node[XP] (twd) at (7,-1) {treewidth + maxdegree$^*$};

% Arrows with bends to avoid crossings
% \draw (diameter) to[bend left=5] (td);
% \draw (diameter) -- (dn);
% \draw (diameter) to[bend left=20]  (nd);
\draw [thick] (cw) -- (tw);
%\draw (cw) to[bend right=10]  (nd);
\draw [thick] (tw) -- (pw);
\draw [thick] (pw) -- (td);
\draw [thick] (tw) -- (fvs);
\draw [thick] (td) -- (vi);
\draw [thick] (vi) -- (vc);
%\draw (tw) to[bend left=18]  (twd);
%\draw (dn) -- (ccn);
\draw [thick] (ccn) -- (dtc);
%\draw (nd) to[bend left=20] (dtc);

\draw [thick] (cw) to[bend right=25] (cvd);
\draw [thick] (cvd) to[bend right=18] (vc);
\draw [thick] (cvd) to[bend left=18] (dtc);
\draw [thick] (fvs) -- (dtp);
\draw [thick] (pw) -- (dtp);
\draw [thick] (fvs) to[bend left=25] (fes);
\draw [thick] (dtp) -- (vc);
%\draw (nd) to[bend right=20]  (vc);

% Legend
% %\node[draw=none, anchor=west] at (6.5,3.5) {\textbf{Complexity Classes:}};
% \node[paraNP, draw=none, anchor=west] at (6.5,4) {paraNP-complete};
% \node[XP, draw=none, anchor=west] at (6.5,3.5) {XP};
% \node[FPTAS, draw=none, anchor=west] at (6.5,3.0) {FPT-AS};
% \node[FPT, draw=none, anchor=west] at (6.5,2.5) {FPT};
\node[paraNP] at (7,3.2) {\textcolor{red!80!black}{paraNP-complete}};
\node[FPT] at (7,2.5) {\textcolor{green!30!black}{FPT}};
%\node[Open] at (7.5,2.6) {Open};
\node[Open] at (7,1.8) {FPT approximable};
%\node[draw, rectangle, sharp corners] at (7.5,3.5) {\textcolor{red!80!black}{paraNP-complete}\\
%%\textcolor{blue}{XP}\\
%%\textcolor{orange}{FPT-AS}\\
%\textcolor{green!30!black}{FPT}\\
%Open
%};

\end{tikzpicture}
}
\caption{Parameterized complexity of {\TB} with respect to structural graph parameters.
The connection between two parameters represents that the upper parameter $p$ is bounded by some
computable function $f(\cdot)$ of the lower parameter $q$, i.e., $p \le f (q)$.
The parameters marked with $*$ are studied in this paper.
The double, rounded, and dotted rectangles indicate paraNP-complete, fixed-parameter tractable, and parameterized approximable cases, respectively.
The exact parameterized complexity of the parameterizations in the last case remains unsettled.
% \tesshu{The current version describes only the related parameters we studied. I'm not sure whether nd and tw + max deg should be included. Also, I'm thinking about how FPT-approximation results should be mentioned. We also should mark pathwidth and treewidth with $^*$?}
%\yota{I changed the description of FPT-approximation results. Please double check.}
}

\label{fig:graph-parameters}
\end{figure}



% \begin{figure}[ht]
% \centering
% \scalebox{0.8}{ % Start scaling
% \begin{tikzpicture}[
%   every node/.style={draw, rectangle, rounded corners, align=center, minimum width=2.8cm, font=\small},
%   paraNP/.style={text=red,draw, rectangle,  double, sharp corners},
%   XP/.style={text=blue, draw, rectangle, sharp corners},
%   FPTAS/.style={text=orange,dash pattern=on 3pt off 2pt},
%   FPT/.style={text=green!50!black},
%   ->, >=Stealth
% ]

% % Nodes positioned to match the original image
% \node[paraNP] (diameter) at (-6.5,4) {diameter};
% \node[paraNP] (dn) at (-6.5,2) {domination number~\cite{tcs/Tale25}};
% \node[FPTAS] (ccn) at (-6.5,-0.5) {clique cover number$^*$};
% \node[FPT] (dtc) at (-6.5,-3.5) {distance to clique$^*$};

% \node[XP] (nd) at (-4,0.5) {neighborhood diversity};


% \node[paraNP] (cw) at (-0.5,4) {cliquewidth};
% \node[paraNP] (tw) at (-0.5,2.5) {treewidth};
% \node[paraNP] (pw) at (-0.5,1) {pathwidth};
% \node[paraNP] (td) at (-0.5,-0.5) {treedepth$^*$};
% \node[FPT] (vi) at (-0.5,-2) {vertex integrity$^*$};
% \node[FPT] (vc) at (-0.5,-3.5) {vertex cover~\cite{tcs/FominFG24}};


% \node[paraNP] (fvs) at (3.5,-0.5) {feedback vertex set};
% \node[paraNP] (dtp) at (3.5,-2) {distance to path forest$^*$ \cite{tcs/Tale25,arxiv/AminianKSS25}};
% \node[FPT] (fes) at (7,-3.5) {feedback edge set~\cite{tcs/FominFG24}};


% \node[XP] (twd) at (7,-1) {treewidth + maxdegree$^*$};

% % Arrows with bends to avoid crossings
% \draw (diameter) to[bend left=5] (td);
% \draw (diameter) -- (dn);
% \draw (diameter) to[bend left=20]  (nd);
% \draw (cw) -- (tw);
% \draw (cw) to[bend right=10]  (nd);
% \draw (tw) -- (pw);
% \draw (pw) -- (td);
% \draw (pw) -- (fvs);
% \draw (td) -- (vi);
% \draw (vi) -- (vc);
% \draw (tw) to[bend left=18]  (twd);
% \draw (dn) -- (ccn);
% \draw (ccn) -- (dtc);
% \draw (nd) to[bend left=20] (dtc);

% \draw (fvs) -- (dtp);
% \draw (fvs) to[bend left=10] (fes);
% \draw (dtp) -- (vc);
% \draw (nd) to[bend right=20]  (vc);

% % Legend
% % %\node[draw=none, anchor=west] at (6.5,3.5) {\textbf{Complexity Classes:}};
% % \node[paraNP, draw=none, anchor=west] at (6.5,4) {paraNP-complete};
% % \node[XP, draw=none, anchor=west] at (6.5,3.5) {XP};
% % \node[FPTAS, draw=none, anchor=west] at (6.5,3.0) {FPT-AS};
% % \node[FPT, draw=none, anchor=west] at (6.5,2.5) {FPT};
% \node[draw, rectangle, sharp corners] at (7.5,3.5) {\textcolor{red}{paraNP-complete}\\
% \textcolor{blue}{XP}\\
% \textcolor{orange}{FPT-AS}\\
% \textcolor{green!50!black}{FPT}
% };

% \end{tikzpicture}
% }
% \caption{Parameterized complexity of {\TB} with respect to structural graph parameters. The connection between two parameters represents that the upper parameter $p$ is bounded by some
% computable function $f(\cdot)$ of the lower parameter $q$, i.e., $p \le f (q)$. The parameters marked with $^*$ are
% studied in this paper.
% \yota{Revised comments to the figure.
% (1) I'm not sure if we could included tw + maxdeg. If we do, we need a proof (or at least a sketch of a proof).
% (2) adding references to the theorems in this paper would be nice.
% (3) clique-width generalizes neighborhood diversity.
% (4) We need to explain what the box shapes mean. Also, it would be nice (for me) if the colors are a little darker.
%  }}
% \label{fig:clean-graph-parameters}
% \end{figure}



==> Sections/fpt_mln.tex <==
\section{Parameterized by Number of Edges or Arcs}

Arguably one of the most natural ways to structurally parameterize \SO\ is to
consider either the number of undirected edges $|E|$ or the number of arcs
$|A|$ as a parameter. Our goal in this section is to investigate the
complexities of these two parameterizations.

We begin with the parameterization by $|E|$, which is trivially FPT: one can
simply guess the orientation of each edge and then check if this gives a valid
solution. The complexity is therefore $2^{|E|}n^{\bO(1)}$. Our contribution is
to observe that this trivial algorithm is perhaps optimal, as if one could
obtain an algorithm of complexity $(2-\varepsilon)^{|E|}n^{\bO(1)}$, then the
Strong Exponential Time Hypothesis (SETH) would be false. Recall that,
informally, the SETH states that there is no algorithm for \textsc{SAT} running
faster than the $2^n$ brute-force algorithm enumerating all assignments. We
show the lower bound by reusing a simple reduction from \textsc{SAT} which
appeared in \cite{ArkinH02}.

\begin{theorem}\label{thm:seth} If there exists an $\varepsilon>0$ such that
\SO\ can be solved in time $(2-\varepsilon)^{|E|}n^{\bO(1)}$, then the
satisfiability of a CNF formula $\phi$ with $n$ variables can be decided in
time $(2-\varepsilon)^n|\phi|^{\bO(1)}$, hence the SETH is false. \end{theorem}

\begin{proof}

Given a CNF formula $\phi$ with variables $x_1,\ldots,x_n$ we construct an
instance of \SO\ with $n$ undirected edges such that the new instance has a
solution if and only if the formula is satisfiable. Clearly, if we perform this
reduction (in polynomial time), then we obtain the theorem.

For each variable $x_i$ of $\phi$ we construct an edge in the new graph, with
one endpoint labeled $x_i$ and the other labeled $\neg x_i$. For each clause
$c$ of $\phi$, suppose that $c$ contains the literals
$\ell_1,\ell_2,\ldots,\ell_p$. We construct two vertices $s_c,t_c$ and the
demand pair $(s_c,t_c)$. We add arcs from $s_c$ to the vertices labeled with
the \emph{negations} of all literals that appear in $c$; and we add arcs from
all vertices labeled with literals that appear in $c$ to $t_c$. This completes
the construction.

Correctness now can be seen as follows. If $\phi$ is satisfiable we orient the
edges so they point towards the true literal of each variable. Each clause $c$
contains a true literal, so there is an arc from $s_c$ to the vertex labeled
with the negation of this literal, then the edge is oriented to the vertex
labeled with the true literal, and then there is an arc to $t_c$, so the demand
$(s_c,t_c)$ is satisfied. For the converse direction, if there is a solution to
the \SO\ instance we extract an assignment to $\phi$ by setting a variable
$x_i$ to true if and only if the edge incident to the vertex labeled $x_i$ is
oriented toward this vertex. We claim this satisfies all clauses. Indeed, if a
clause $c$ were \emph{not} satisfied, this means that all edges are oriented
towards vertices labeled with the negations of the literals of $c$. This
implies that the demand $(s_c,t_c)$ is not satisfied, because any path starting
from $s_c$ must move towards a vertex labeled with the negation of a literal of
$c$ and since the undirected edges cannot be used to exit such a vertex we
cannot reach $t_c$. We conclude that we have a satisfying assignment of $\phi$.
\end{proof}

The main result of this section is then to establish that the parameterization
by $|A|$ also gives a fixed-parameter tractable problem, and indeed that we are
again able to obtain a single-exponential parameter dependence. This
parameterization is significantly more challenging, so we will need to rely on
structural properties obtained by any graph where $|A|$ is small after we apply
some simple reduction rules. The main result we obtain is stated below.

\begin{theorem}\label{thm:arcs} \SO\ admits a $2^{\bO(|A|)}n^{\bO(1)}$ algorithm.
\end{theorem}

Our high-level strategy will be made up of two parts. First, we define a (very)
restricted special case of \SO, where, notably, all undirected components are
paths (and we have some additional restrictions). Despite the severe
restrictions, this case is still not trivial. In particular, the instances constructed in \cref{thm:seth} are instances of this special case, so this restriction is still NP-hard. However, we will be able to show that
it admits an FPT algorithm with running time $2^cn^{\bO(1)}$, where $c$ is the
number of undirected components, via a reduction to \textsc{2-SAT}. Second, we
will show how a branching procedure can reduce any initial instance into a
collection of at most $2^{\bO(|A|)}$ instances of the restricted problem, each
having $\bO(|A|)$ undirected components. The result will then follow by composing
the two algorithms. The key intuition of the second part will be that bounding $|A|$ also bounds the feedback edge set of the underlying graph, that is, the number of edges we need to delete to destroy all cycles. In order to ease presentation, we start with the algorithm
for the restricted case in \cref{sec:paths} and then give the algorithm for parameter $|A|$
in \cref{sec:arcs}.

\subsection{A Restricted Case}\label{sec:paths}

We define a restricted case of \SO\ as follows:

\begin{definition}\label{def:restricted} An instance $G=(V,E,A)$ of \SO\ is
called \emph{restricted} if we have the following: (i) all vertices $v\in V$
are incident on at most $2$ edges of $E$ (ii) all vertices $v\in V$ which are
incident on exactly $2$ edges of $E$ are incident on no arcs of $A$.
\end{definition}

Intuitively, a restricted instance which is also mixed acyclic is an instance
where each undirected component is a path (because the maximum degree induced
by $E$ is $2$ and we have no cycles) and furthermore the internal vertices of
each such path have no arcs connecting them to the outside. We remark here that in the instances constructed in \cref{thm:seth} all vertices are incident on at most $1$ undirected edge, so the constraints of \cref{def:restricted} are satisfied, hence this restriction is still NP-hard. 

Our strategy to handle restricted instances of \SO\ will be the following:
first, we guess whether there are any undirected components (paths) where all
the edges must be oriented in the same direction and orient such paths
accordingly. We then arrive in a situation where we are looking for a solution
where the undirected paths will be oriented in such a way that it will be
impossible to reach one endpoint from the other. This allows us to encode our
instance as a \textsc{2-SAT} formula, by defining for each internal vertex a
variable which encodes whether this vertex can reach one endpoint of its path
or the other in the final solution or whether this vertex can be reached by one
endpoint or the other.

\begin{lemma}\label{lem:restricted} There is an algorithm that takes a
restricted \SO\ instance $G=(V,E,A)$ that is mixed acyclic and decides if a
solution exists in time $2^{O(c)}n^{\bO(1)}$, where $c$ is the number of
connected components of $G[E]$.  \end{lemma}

\begin{proof}

We begin with some simple observations. First, if we have a restricted \SO\
instance $G=(V,E,A)$ and we orient an undirected edge, that is, we produce a
new instance $G'=(V,E',A')$ by selecting an edge $e=\{u,v\}\in E$ and setting
$E'=E\setminus\{e\}$ and $A'=A\cup \{\ (u,v)\ \}$ or $A'=A\cup\{\ (v,u)\ \}$,
then the new instance is still restricted. This will be useful as we will
attempt to solve the given instance via a branching algorithm that orients some
edges of $E$.

Let $P_1,P_2,\ldots,P_c$ be the components of $G[E]$, which all induce
(possibly trivial) paths, as the instance is mixed acyclic and has maximum
degree $2$ in undirected edges. Suppose that there exists a demand pair $(s,t)$
such that $s,t\in P_i$, for some $i\in[c]$. Then, there is a unique way to
satisfy this pair (as the graph is mixed acyclic), so we orient the edges of
$P_i$ connecting $s$ to $t$ appropriately and obtain a simpler instance. In the
remainder we assume that for each demand pair $(s,t)$ we have that $s\in P_i$,
$t\in P_j$ and $i<j$, which we can achieve by topologically sorting the
components.

We say that an orientation of the edges of a component $P_i$ is \emph{uniform}
if the orientation creates a directed path from one endpoint of $P_i$ to the
other. The first step of our algorithm is to guess for which components $P_i$
the solution uses a uniform orientation and guess for these components the
direction of the orientation. We have at most $3^c$ choices, which produce
$3^c$ new restricted instances of \SO. We now have that: (i) if the original
instance has a solution, then one of the new instances has a solution which
\emph{never} uses a uniform orientation on any non-trivial component $P_i$ (ii)
if one of the new instances has a solution (uniform or not), the original one
does as well.

We will now reduce the problem to \textsc{2-SAT} in a way that if a solution
avoiding uniform orientations exists, the new instance is satisfiable; while if
the new instance is satisfiable we can find some orientation satisfying all
demands. This will be sufficient to solve the original instance.  We mention
that we will no longer assume that the number of components $P_i$ is bounded by
$c$ (as orienting a path has the effect of creating many trivial components in
$G[E]$), but this is not a problem as we are now reducing to a polynomial-time
(rather than FPT) solvable problem.  Note also that, because when a component
$P_i$ has exactly two vertices all its orientations are trivially uniform, we
can assume we have an instance where all non-trivial components have at least
$3$ vertices.

For each non-trivial component $P_i$ of $G[E]$ (that is, each component made up
of at least $3$ vertices) we arbitrarily pick one endpoint of $P_i$ to be the
left endpoint and call the other endpoint the right endpoint. For each
\emph{internal} vertex $v\in P_i$ we define four variables $x_{v\to L}, x_{v\to
R}, x_{L\to v}, x_{R\to v}$, whose informal meaning should be understood as
``if this variable is true, then the solution contains a directed path from $v$
to the left (respectively right) endpoint of $P_i$'' or ``if this variable is
true, then the solution contains a directed path from the left (respectively
right) endpoint of $P_i$ to $v$''.  Furthermore, for each edge $e\in E$ we
construct variables $y_{e\to L}$, $y_{e\to R}$ whose informal meaning is ``in
the solution, edge $e$ is oriented towards the left (respectively right)
endpoint of its path''.

We now construct a \textsc{2-SAT} instance as follows:

\begin{enumerate}

\item (Basic Consistency Clauses): For each edge $e\in E$ we add the clause
$(\neg y_{e\to L}\lor \neg y_{e\to R})$.

\item (Pair Consistency clauses): For each non-trivial component $P_i$,  each
internal vertex $v\in P_i$ and each edge $e\in P_i$ we do the following: if $e$
is in the path from $v$ to the left endpoint we add the clauses $(x_{v\to L}\to
y_{e\to L})$ and $(x_{L\to v}\to y_{e\to R})$; otherwise we add the clauses
$(x_{v\to R}\to y_{e\to R})$ and $(x_{R\to v}\to y_{e\to L})$.


\item (Basic Terminal clauses): For each terminal pair $(s,t)$ such that $s$ is
an internal vertex of $P_i$ we add the clause $(x_{s\to L}\lor x_{s\to R})$.
Similarly, for each terminal pair $(s,t)$ such that $t$ is an internal vertex
of a path $P_i$ we add the clause $(x_{L\to t}\lor x_{R\to t})$.

\end{enumerate}

The clauses we have constructed so far encode the basic structure of the
instance. What remains is to add clauses ensuring that we must orient edges in
a way that satisfies all demands. In the remainder, when we say that $v$ is an
endpoint of the component $P_i$ of $G[E]$ we mean that either $P_i$ is a path
and $v$ is one of its endpoints or that $P_i$ is trivial (that is, $v$ is
isolated in $G[E]$). For each demand pair $(s,t)$ we do the following:

\begin{enumerate}

\item If $s,t$ are both endpoints of their components, we check if there is a
directed path from $s$ to $t$ in $G[A]$. If this is the case we remove the
demand pair $(s,t)$, as it is already satisfied. Otherwise we reject the
current instance as this demand cannot be satisfied.

\item If $s$ is an endpoint of its component but $t$ is an internal vertex of
$P_i$ we check if there is a directed path in $G[A]$ from $s$ to the left
(respectively right) endpoint of $P_i$. If no such path exists, we add to the
instance the clause $\neg x_{L\to t}$ (respectively $\neg x_{R\to t}$).

\item Symmetrically to the previous step, if $s$ is an internal vertex of $P_i$
and $t$ an endpoint, we check if $G[A]$ has a path from the left (respectively
right) endpoint of $P_i$ to $t$. If no such path exists, we add to the instance
the clause $\neg x_{s\to L}$ (respectively $\neg x_{s\to R}$).

\item Finally, if $s$ is an internal vertex of $P_i$ and $t$ an internal vertex
of $P_j$ we check whether $G[A]$ contains a directed path from each endpoint of
$P_i$ to each endpoint of $P_j$. If $G[A]$ contains no path from the left
endpoint of $P_i$ to the left endpoint of $P_j$ we add the clause $(\neg
x_{s\to L}\lor \neg x_{L\to t})$; similarly, if there is no path from the left
endpoint of $P_i$ to the right endpoint of $P_j$ we add the clause $(\neg
x_{s\to L}\lor \neg x_{R\to t})$; we add the clause $(\neg x_{s\to R}\lor \neg
x_{L\to t})$ if there is no path from the right endpoint of $P_i$ to the left
endpoint of $P_j$; and the clause $(\neg x_{s\to R}\lor \neg x_{R\to t})$ for
the remaining case.

\end{enumerate}

This completes the construction and we now need to argue for correctness. Let
us then start with a useful claim.

\begin{claim} Let $x,y$ be two endpoints of $G$ such that $G[A]$ has no
directed path from $x$ to $y$. Then, it is impossible to construct a directed
path from $x$ to $y$ without uniformly orienting a component $P_i$ of $G[E]$.
\end{claim}

\begin{claimproof} The claim is not hard to see, because a non-uniform
orientation of $P_i$ does not add a directed path between the endpoints of
$P_i$, hence any set of orientation will add no directed path between any two
endpoint vertices.  \end{claimproof}

Armed with the claim above we can then see that the unique case where our
algorithm directly rejects the instance (when $(s,t)$ is a demand pair with
$s,t$ endpoints but no path from $s$ to $t$ in $G[A]$) is correct. We will then
focus on the case where this did not happen, so a \textsc{2-SAT} instance is
produced and we want to show that this instance allows us to decide the given
\SO\ instance.

For one direction, suppose that there exists an orientation satisfying all
demand pairs. We assign values to the edge variables according to their
informal meanings. Furthermore, for each demand pair $(s,t)$ pick a directed
path in the solution that connects $s$ to $t$. If $s$ is internal and the path
goes through the left endpoint of its path set $x_{s\to L}$ to true, otherwise
set $x_{s\to R}$ to true and act similarly for $t$. Set all remaining variables
to false.  

We observe that the Basic Consistency clauses, Pair Consistency clauses, and
Basic Terminal clauses are clearly satisfied by this assignment. Furthermore,
the clauses we added to encode terminal pairs are also satisfied. To see this,
suppose that a demand pair $(s,t)$, where $s,t$ are internal vertices, is
satisfied by a path going through the left endpoints of the respective paths,
so $x_{s\to L}, x_{L\to t}$ are true and $x_{s\to R}, x_{R\to t}$ are false.
According to the claim, this means that the left endpoints already have a
directed path in $G[A]$, hence we did not add the clause $(\neg x_{s\to L}\lor
\neg x_{L\to t})$, which is the only clause that would have been falsified in
this case. The other cases are similar and the case where one of $s,t$ is
internal is also similar (and simpler).

For the converse direction, we claim that if the resulting instance has a
satisfying assignment, we can find a valid orientation of $E$ to satisfy all
demands. Indeed, we can extract an orientation by examining the values of the
variables $y_{e\to L}, y_{e\to R}$, which thanks to the basic consistency
clauses assign at most one orientation to each edge (if both variables are
false, orient $e$ arbitrarily). We now claim that the informal meaning of the
remaining variables is preserved, meaning that when $x_{v\to L}$ is true, then
the orientation does have a path from $v$ to the left endpoint of the path
containing $v$. This is implied by the pair consistency clauses, and similarly
holds for $x_{v\to R}, x_{L\to v}, x_{R\to v}$. Consider now a demand $(s,t)$
and by the basic terminal clauses we have one of $x_{s\to L}, x_{s\to R}$ true
and one of $x_{L\to t}, x_{R\to t}$ true. Suppose $x_{s\to L}, x_{L\to t}$ are
true (the other cases are symmetric). We claim that there must be path from $s$
to $t$ in the orientation using the left endpoints of the paths containing
$s,t$, as otherwise we would have added the clause $(\neg x_{s\to L}\lor \neg
x_{L\to t})$.  

This completes the reduction and since \textsc{2-SAT} can be solved in
polynomial time we obtain the lemma.  \end{proof}

\subsection{FPT algorithm by Number of Arcs}\label{sec:arcs}

\begin{proof}[Proof of \cref{thm:arcs}]

We begin by applying \cref{prop:prepoc} and \cref{prop:remove:degree:1}
exhaustively. This does not increase $|A|$, so we can assume that the
input is mixed acyclic and has no vertices of degree at most $1$. Our algorithm
is now the following: as long as the current instance is not restricted (in the
sense of \cref{def:restricted}), we select a vertex $v$ which violates the
constraints, preferring a vertex that violates the first constraint, if possible. Such a vertex must necessarily be incident on at least one
undirected edge $e\in E$. Pick such an edge $e$ and try out both orientations
of $e$, producing two new instances. We claim that in the end we will obtain
$2^{\bO(|A|)}$ restricted instances, such that at least one of them will have a solution if
and only if the original instance did. Furthermore, all instances will have at most $\bO(|A|)$ undirected components.

In order to establish this claim, we want to show that the branching depth is
bounded by $\bO(|A|)$, that is, branching on $\bO(|A|)$ edges is always sufficient to arrive at a restricted instance. Consider then the undirected graph   $G[E]$. For each
integer $i$, let $n_i$ be the number of vertices of degree $i$ in $G[E]$. We have
$n_1\le 2|A|$, because the original instance has no degree $1$ vertices (by
applying \cref{prop:remove:degree:1}), so any leaf of $G[E]$ must be incident on
an arc of $|A|$. 
Furthermore, we have that $\sum_{i} i\cdot
n_i \le 2n-2$, because $G[E]$ is a forest and the sum of degrees is equal to twice
the number of edges. Manipulating, we have $\sum_{i\ge 3} i\cdot n_i + 2n_2 +
n_1 \le 2n-2 \Leftrightarrow \sum_{i\ge 3}(i-2)n_i + 2n - n_1 \le 2n-2
\Rightarrow \sum_{i\ge 3}(i-2)n_i \le 2|A|$. 

We now observe that the above analysis implies that the branching depth of our
algorithm is $\bO(|A|)$. More precisely, suppose that we first branch on vertices that violate the first property of \cref{def:restricted} as long as this is possible. For a vertex $v$ that has degree $i$ in $G[E]$ we will branch $(i-2)$ times to make it satisfy the first property. But we argued that $\sum_{i\ge 3} (i-2)n_i\le 2|A|$, so this part has linear branching depth. Then, as long as all vertices satisfy the first property, we pick a vertex that violates the second property and branch on one of its incident edges. This will happen at most once per vertex. Because each vertex we branch on must either be incident on an original arc (there are at most $2|A|$ such vertices) or incident on an arc we created in the first branching part by orienting an edge (there are at most $4|A|$ such vertices), the second branching part has depth at most $6|A|$. So, the total branching depth is $\bO(|A|)$.

From the above analysis we conclude that we can produce $2^{\bO(|A|)}$ instances
on which we can invoke \cref{lem:restricted}. However, we also need to argue
that the number of connected components of $G[E]$ in these
instances is $\bO(|A|)$. To see this, observe that if the original graph was weakly connected (we assume this without loss of generality), then we had at most $|A|$ undirected components in $G[E]$ initially. Orienting an edge can only increase the number of undirected components by $1$, so since we perform a branching algorithm which in each branch orients at most $\bO(|A|)$ edges, in the end we have at most $\bO(|A|)$ undirected components.
\end{proof}

%----
%
%\begin{theorem}
%    We can decide if $(G, \terminals)$ is a yes instance of \SO\ in FPT time parameterized by $|A(G)|$ or $\fes(\hat{G})$ or $\hat{G}$ or $\ml(\hat{G})$, where $\hat{G}$ the underlying graph of $G$.
%\end{theorem}
%
%\begin{proof}
%
%    First, we show that it suffices to design an FPT algorithm parameterized by the max leaf number, $\ml$, of $\hat{G}$.
%    
%    Recall that we may assume that $G$ contains no mixed cycles \textcolor{red}{[reference]} and no vertices of degree~1 \textcolor{red}{[reference]}. We prove that any such graph satisfies $\ml(\hat{G}) \le 2\fes(\hat{G}) \le 2|A(G)|$.
%    
%    To prove the first inequality, we use the fact that any spanning tree of $\hat{G}$ has exactly $|E(\hat{G})| - \fes(\hat{G})$ edges, and that $\hat{G}$ has no vertices of degree~1. By definition of the max leaf number, $\hat{G}$ has a spanning tree with $\ml(\hat{G})$ leaves. This tree is missing exactly $\fes(\hat{G})$ edges from $E(\hat{G})$. Since removing $\fes(\hat{G})$ edges can create at most $2\fes(\hat{G})$ new vertices of degree~1, and since $\delta(\hat{G}) \ge 2$, we conclude that $\ml(\hat{G}) \le 2\fes(\hat{G})$.
%    
%    To prove the second inequality, we use the fact that $G$ contains no cycles, which implies that $G - A$ is a forest. Therefore, $\fes(\hat{G}) \le |A(G)|$.
%    
%    Given these inequalities, it suffices to prove that the problem is FPT when parameterized by the max leaf number of $\hat{G}$. The algorithm proceeds as follows:
%    \begin{itemize}
%        \item First, generate an FPT number of instances by guessing orientations of certain edges
%        \item Then identify properties of potential paths between terminal pairs under the assumption of correct guesses
%        \item Finally, model the problem as a 2-SAT instance using these properties
%    \end{itemize}
%    Since the number of instances is FPT and 2-SAT is solvable in polynomial time, we obtain an FPT algorithm.
%
%
%
%    \proofsubparagraph{Guessing and creating the new instances}
%    We begin by considering the underlying graph $\hat{G}$ of $G$. Also, let $\ml$ be the max-leaf number of $\hat{G}$.
%    
%    It is known that any graph with max-leaf number $\ml$ can be obtained from a simple graph $H$ (i.e., without parallel edges or loops) of order $O(\ml)$ by edge subdivisions. Moreover, we may assume such a graph $H$ is given; otherwise, it can be computed in FPT time~\cite{KleitmanW91}.
%    
%    Let $U \subseteq V$ be the vertices of $\hat{G}$ appearing in $H$. Between any two vertices $u,v \in U$, there exists at most one $u$-$v$ path in $\hat{G}$ using only vertices from $V \setminus U$ as intermediate vertices (otherwise, $H$ would not be simple). Let $P_1, P_2, \ldots, P_\ell$ be all such paths in $G$, including paths of length 1 (i.e., edges $\{u,v\} \in E(\hat{G})$). Note that $\ell < \ml^2$ since the number of such paths is bounded by the number of edges in $H$.
%    
%    For each path $P_i$, $i \in [\ell]$, we first guess whether all edges in $P_i$ share the same direction in the final orientation. If yes, we also guess the common direction. If no, we guess only the directions of the first and last edges in $P_i$. This results in at most $6^\ell < 6^{\ml^2}$ total guesses.
%    
%    We can verify (in polynomial time) whether a guess agrees with set $A$, discarding those that do not. 
%    Notice that, since we consider all possible guesses, if the instance is a yes-instance of \textsc{Steiner Orientation}, at least one guess will agree with an orientation where all terminal pairs are connected. Henceforth, we assume we are working with such a correct guess.
%    
%    Let $E' \subseteq E(\hat{G})$ be the set of edges whose orientations we have guessed, and let $\hat{A}^*$ be the set of arcs obtained by orienting the edges in $E'$ according to our guesses.  Also let $\hat{E}^*$ be the set of edges that remains undirected; i.e., $\hat{E}^*=  E(\hat{G}) \setminus E'$. Notice that there is not direct relation between $\hat{E}^*$ and $E(G)$.
%    %Finally, let $\hat{G}^* =  (V, \hat{E},A\cup \hat{A}^*)$.
%    
%
%    %% maybe it not needed:
%    
%        %Let $E' \subseteq E(\hat{G})$ be the set of edges whose orientations we have guessed, and let $\hat{A}^*$ be the set of arcs obtained by orienting the edges in $E'$ according to our guesses.  
%        %Let $\hat{G}^* = (V, \overline{E}^*, \hat{A}^*)$ be the mixed graph obtained from $\hat{G}$ after applying these guesses, and let $G^* = (V, E^*, A^*)$ be the mixed graph obtained from $G$ after applying the guesses to the edges in $E' \cap E(G)$.
%
%
%    \proofsubparagraph{Properties of $s$-$t$ paths in $\hat{G}^*$}
%
%
%    Before analyzing the properties of $s$-$t$ paths, we first define a new set of paths in $\hat{G}^*$. 
%    In particular, notice that the edge set $\overline{E}^*$ defines a collection of undirected paths in $\hat{G}^*$. 
%    \textcolor{red}{Is the previous clear? Our earlier guesses ensure that any edge incident to a vertex of degree $\geq 3$ has been converted to an arc.} 
%    Each such path is a sub-path of some path $P_i$, $i \in [\ell]$, in $\hat{G}$. Also, since we guessed the orientations of the first and last edges of each $P_i$, we have $V(\overline{E}^*) \subseteq V \setminus U$.
%    
%    Assuming correct guesses, there exists an orientation of $\hat{G}^*$ (consistent with $A$) where for every terminal pair $(s,t)$, an $s$-$t$ path $P_{s,t}$ exists. 
%    Note that, under the current guesses, some edges of $P_{s,t}$ remain undirected (i.e., belong to $\overline{E}^*$). 
%    This leads to the following key observation:
%    
%    \begin{observation}\label{obs:form:of:paths:for:variable:vertices}
%    The edges of $P_{s,t}$ in $\hat{G}^*$ can be partitioned into three (possibly empty) subpaths:
%    \begin{itemize}
%        \item $P_{s,t}^1$ and $P_{s,t}^3$: Undirected subpaths ($E(P_{s,t}^1) \cup E(P_{s,t}^3) \subseteq \overline{E}^*$)
%        \item $P_{s,t}^2$: A directed subpath in $\hat{G}^*$
%    \end{itemize}
%    such that $P_{s,t} = P_{s,t}^1 - P_{s,t}^2 - P_{s,t}^3$.
%    \end{observation}
%    
%    The observation holds because we correctly guessed which paths $P_i$ have uniformly oriented edges in the final orientation. 
%    Therefore, if $P_{s,t}$ enters an undirected path in $\hat{G}^*$ but exits from the opposite end, this would imply all edges in that path share the same direction. This contradicts the assumption that we are considering a correct guess.
%    
%    Using these observations, we now formulate the problem as a 2-SAT instance.
%
%    \proofsubparagraph{Reduction to $2$-SAT}
%    
%    By Observation~\ref{obs:form:of:paths:for:variable:vertices} we know that, if we have a yes-instance and have made the correct guesses, the path between $s$ and $t$ consists of edges in $\overline{E}^*$, followed by arcs in $\hat{A}^*$, and then edges in $\overline{E}^*$ again. 
%    Because of this structure, we can conclude that the (currently) undirected edges appearing in the $s$-$t$ path must belong to the paths containing $s$ and $t$ in $(V,\overline{E}^*)$. 
%    
%    At a high level, this gives two options for $s$ and two options for $t$ (i.e., which endpoint of their respective paths will be used in the $s$-$t$ path we are searching for).
%    Additionally, each edge in $\overline{E}^*$ has two possible orientations. The direction of the $s$-$t$ paths must agree with these edge orientations.
%    
%    We model this as a 2-SAT instance, splitting the process into two steps:
%    
%    \textbf{Step 1 (handling edges):} We create variables and clauses related to edges. In particular, we create:
%    \begin{itemize}
%        \item ``Edge variables'': Represent the two possible directions for each undirected edge
%        \item ``Edge clauses'': Enforce that our solution agrees with the original arc set $A$
%    \end{itemize}
%    
%    \textbf{Step 2 (handling terminal pairs):} We create variables and clauses related to terminal pairs. In particular, we create:
%    \begin{itemize}
%        \item ``Terminal variables'': Represent which part of their path each terminal will use for the potential $s$-$t$ path
%        \item ``Path orientation clauses'': Force terminal variables to agree with edge variables (to enable path formation)
%        \item ``Directed path clauses'': Allow only specific combinations of values per pair of terminal variables (based on available directed paths)
%    \end{itemize}
%    
%    \subparagraph{Step 1:}
%    The first step is to create variables that represent the possible orientations for undirected edges in $\overline{E}^*$.
%    
%    To properly define these variables, we first (arbitrarily) select a positive and negative direction for each maximal undirected path $P$ in $(V,\overline{E}^*)$. Specifically, we fix which vertex is considered first and which is last. Hereafter, for any maximal path $P$ in $(V,\overline{E}^*)$, we assume that $u^P_{first}$ and $u^P_{last}$ are the starting and ending vertices of $P$ respectively. If a path consists of an isolated vertex $v$, we set $u^P_{first} = u^P_{last} = v$.
%    
%    Consider an edge $e = \{u,v\}$ of $P$ where the distance between $u$ and $u^P_{last}$ in $P$ is smaller than the distance between $v$ and $u^P_{last}$ in $P$. We then define the arc $(u,v)$ as the positive orientation of $e$ and $(v,u)$ as the negative orientation. Note that paths consisting of isolated vertices contain no edges, so this definition remains consistent.
%    
%    For each edge $e \in \overline{E}^*$, we create a variable $x_e$ representing its possible orientations. This variable determines the edge's direction: when $x_e = true$ we select the positive orientation, and when $x_e = false$ we select the negative orientation.
%    
%    Some edges in $\overline{E}^*$ may correspond to arcs in $A$. The selected orientation for these edges must agree with $A$. Therefore, if edge $e$ is oriented positively in $A$, we add the clause $(x_e)$. Similarly, if $e$ is oriented negatively in $A$, we add the clause $(\neg x_e)$. We call these clauses \textit{edge clauses}.
%
%    \subparagraph{Step 2:}
%    We partition the terminal pairs into two sets. Let $\terminals_1$ be the set of terminal pairs $(s,t)$ where both $s$ and $t$ belong to the same path in $(V,\hat{E}^*)$, and let $\terminals_2 = \terminals \setminus \terminals_1$. For any $(s,t)\in \terminals_2$, $s$ and $t$ belong to different paths in $(V,\hat{E}^*)$.
%    
%    We handle each set separately. First, for $\terminals_1$, we create variables $y_s$ and $y_t$ for each $(s,t)\in \terminals_1$. These variables represent the direction the $s$-$t$ path uses in their shared path $P$ of $(V,\hat{E}^*)$. Since $s$ and $t$ are in the same path $P$, the $s$-$t$ path either uses only edges in $P$ or leaves $P$ from one end, uses edges of $\hat{A}^*$, and enters from the other end to reach $t$. This implies $y_s = y_t$, which we enforce by adding the clauses $(\neg y_s \lor y_t)$ and $(\neg y_t \lor y_s)$ in $\phi$.
%    
%    To orient the edges correctly, we first partition the edges of $P$ into three sets. Let $u^s$ be the vertex in $\{u^P_{first}, u^P_{last}\}$ that is closer to $s$ than $t$, and let $u^t$ be the remaining vertex. We define $E^s$ as the edges connecting $s$ and $u^s$ in $P$, $E^{s,t}$ as the edges connecting $s$ and $t$ in $P$, and $E^t$ as the edges connecting $t$ and $u^t$ in $P$.
%    
%    The clauses we add depend on whether $u^s = u^P_{first}$ or not. 
%    
%    \textbf{Case 1} ($u^s = u^P_{last}$): If $y_s = y_t = true$, we connect $s$ and $t$ using edges of $E^{s,t}$ by adding $(\neg y_s \lor x_e)$ for all $e\in E^{s,t}$. If $y_s = y_t = false$, we orient edges of $E^s$ from $s$ to $u^P_{first}$ and edges of $E^t$ from $u^P_{last}$ to $t$ by adding $(y_s \lor x_e)$ for all $e\in E^s \cup E^t$. When no path in $\hat{A}^*$ connects $u^P_{last}$ and $u^P_{first}$, we add $(y_s)$ to prevent $y_s = y_t = false$.
%    
%    \textbf{Case 2} ($u^s = u^P_{first}$): The arguments are symmetric with directions reversed. If $y_s = y_t = false$, we add $(y_s \lor \neg x_e)$ for all $e\in E^{s,t}$. If $y_s = y_t = true$, we add $(\neg y_s \lor x_e)$ for all $e\in E^s \cup E^t$. Similarly, if no path in $\hat{A}^*$ connects $u^P_{first}$ and $u^P_{last}$, we add $(\neg y_s)$ to prevent $y_s = y_t = true$.
%    
%    We repeat this process for all pairs in $\terminals_1$.
%    
%    Now, we consider terminal pairs $(s,t)\in \terminals_2$. Notice that in this case, $s$ and $t$ belong to different paths in $(V,\overline{E}^*)$. Let $P$ and $Q$ be the maximal paths of $(V,\overline{E}^*)$ where $s$ and $t$ belong, respectively. We create variables $x_s$ and $x_t$, where $x_s$ indicates the direction from which the $s$-$t$ path leaves path $P$, and $x_t$ indicates the direction from which it enters path $Q$. We need to orient the edges in $P$ and $Q$ consistently with these variable assignments.
%    
%    First we consider the edges of $P$. Let $E_{first}^s$ be the edges between $u_{first}^P$ and $s$ (which may be empty if $u_{first}^P=s$), and $E_{last}^s$ be the edges between $u_{last}^P$ and $s$ (which may be empty if $u_{last}^P=s$). The $s$-$t$ path either uses all edges in $E_{first}^s$ in their positive direction or all edges in $E_{last}^s$ in their negative direction. Therefore, when $x_s=true$ we require $x_e=true$ for all $e\in E_{first}^s$, enforced by adding clauses $(\neg x_s \lor x_e)$ for all $e\in E_{first}^s$. When $x_s=false$ we require $x_e=false$ for all $e\in E_{last}^s$, enforced by adding clauses $(x_s \lor \neg x_e)$ for all $e\in E_{last}^s$.
%    
%    Similarly for path $Q$, let $E_{first}^t$ be the edges between $u_{first}^Q$ and $t$ (possibly empty if $u_{first}^Q=t$), and $E_{last}^t$ be the edges between $u_{last}^Q$ and $t$ (possibly empty if $u_{last}^Q=t$). The $s$-$t$ path either uses all edges in $E_{first}^t$ negatively or all edges in $E_{last}^t$ positively. Therefore, when $x_t=true$ we require $x_e=true$ for all $e\in E_{last}^t$, enforced by adding clauses $(\neg x_t \lor x_e)$ for all $e\in E_{last}^t$. When $x_t=false$ we require $x_e=false$ for all $e\in E_{first}^t$, enforced by adding clauses $(x_t \lor \neg x_e)$ for all $e\in E_{first}^t$.
%
%    Notice that this does not yet guarantee that the terminals $s$ and $t$ can be connected. In particular, we also need to check which of the following paths exist in $(V,\hat{A}^*)$: 
%    \begin{enumerate}[(i)]
%        \item \label{path1} $u_{first}^P$ - $u_{first}^Q$,  
%        \item $u_{first}^P$ - $u_{last}^Q$,  
%        \item $u_{last}^P$ - $u_{first}^Q$ and 
%        \item $u_{last}^P$ - $u_{last}^Q$.   
%    \end{enumerate}
%    
%    Notice that the absence of any of these paths forces us to consider particular values for the variables $x_s$ and $x_t$. For this reason, we add extra clauses to our 2-SAT formula $\phi$ according to these rules:
%    
%    \textbf{Rule 1.} If none of the paths exist: then we have a no-instance and we can stop.
%    
%    \textbf{Rule 2.} If neither (i) nor (ii) exists: then $x_s=false$ since we can only connect $s$ and $t$ via $u_{last}^P$. Therefore we add the clause $(\neg x_s)$ in $\phi$. This does not directly imply anything for $x_t$.
%    
%    \textbf{Rule 3.} If neither (iii) nor (iv) exists: then $x_s=true$ since we can only connect $s$ and $t$ via $u_{first}^P$. Therefore we add the clause $(x_s)$ in $\phi$. This does not imply any restrictions for $x_t$.
%    
%    \textbf{Rule 4.} If neither (i) nor (iii) exists: then $x_t=true$ since we can only connect $s$ and $t$ via $u_{last}^Q$. Therefore we add the clause $(x_t)$ in $\phi$. This does not imply any restrictions for $x_s$.
%    
%    \textbf{Rule 5.} If neither (iii) nor (iv) exists: then $x_t=false$ since we can only connect $s$ and $t$ via $u_{first}^Q$. Therefore we add the clause $(\neg x_t)$ in $\phi$. This does not imply any restrictions for $x_s$.
%    
%    Now we check whether any values for $x_s$ force the value of $x_t$ and vice versa:
%    
%    \textbf{Rule 6.} If exactly one of (i) and (ii) exists: then when $x_s=true$ we have a unique value for $x_t$. If only (i) exists then $x_s=true$ requires $x_t=false$, so we add $(\neg x_s \lor \neg x_t)$ to $\phi$. If only (ii) exists then $x_s=true$ requires $x_t=true$, so we add $(\neg x_s \lor x_t)$ to $\phi$. These impose no restrictions when $x_s=false$.
%    
%    \textbf{Rule 7.} If exactly one of (iii) and (iv) exists: then when $x_s=false$ we have a unique value for $x_t$. If only (iii) exists then $x_s=false$ requires $x_t=false$, so we add $(x_s \lor \neg x_t)$ to $\phi$. If only (iv) exists then $x_s=false$ requires $x_t=true$, so we add $(x_s \lor x_t)$ to $\phi$. These impose no restrictions when $x_s=true$.
%    
%    \textbf{Rule 8.} If exactly one of (i) and (iii) exists: then when $x_t=false$ we have a unique value for $x_s$. If only (i) exists then $x_t=false$ requires $x_s=true$, so we add $(x_s \lor x_t)$ to $\phi$. If only (iii) exists then $x_t=false$ requires $x_s=false$, so we add $(\neg x_s \lor x_t)$ to $\phi$. These impose no restrictions when $x_t=true$.
%    
%    \textbf{Rule 9.} If exactly one of (ii) and (iv) exists: then when $x_t=true$ we have a unique value for $x_s$. If only (ii) exists then $x_t=true$ requires $x_s=true$, so we add $(x_s \lor \neg x_t)$ to $\phi$. If only (iv) exists then $x_t=true$ requires $x_s=false$, so we add $(\neg x_s \lor \neg x_t)$ to $\phi$. These impose no restrictions when $x_t=false$.
%
%    We repeat this process for all terminal pairs in $\terminals_2$.
%    
%    Notice that the clauses containing both terminal variables and edge variables ensure that we correctly orient the undirected edges of $\overline{E}^*$. We call these clauses \textit{path orientation clauses}. 
%    
%    The clauses containing only terminal variables ensure that the selected combination for each terminal pair is valid, meaning the required directed paths exist to form these connections. These clauses are called \textit{directed path clauses}.
%        
%    \proofsubparagraph{Correctness} Notice that, if we have started with a yes instance of \textsc{Steiner Orientation}, then there exists a guess that agrees with an orientation $\overrightarrow{E}$ of $E$ such that, in $(V,A\cup \overrightarrow{E})$, for every terminal pair $(s,t)\in \terminals$ there exists an $s$-$t$ path. Then the restrictions we have imposed imply that:
%    \begin{itemize}
%        \item We orient the edges uniquely (each edge is related to an edge variable),
%        \item We orient the edges in a way that allows paths to be formed (forced by the path orientation clauses), and
%        \item We are not considering non-existing paths (forced by the directed path clauses).
%    \end{itemize}  
%    Notice that all the clauses we have added must be satisfied if we have uniquely oriented all edges and all $s$-$t$ paths exist in the final orientation. 
%    Therefore, the 2-SAT instance we created (under the guess that agrees with $\overrightarrow{E}$) is a yes instance.
%    
%    
%    It remains to prove that if at least one of the created 2-SAT instances is a yes-instance, then the original \textsc{Steiner Orientation} instance is a yes-instance. Assume we have a yes-instance of 2-SAT, and let $D$ be the orientation of $G$ that agrees with both our guesses and the values of the edge variables $x_e$. Note that the edge clauses we added during Step 1 ensure this orientation agrees with $A$, guaranteeing $D$ is indeed a valid orientation of $G$.
%    
%    We claim that for every terminal pair $(s,t)\in \terminals$, there exists an $s$-$t$ path in $D$. Observe that for each pair, either both $y_s$ and $y_t$ or both $x_s$ and $x_t$ appear in the 2-SAT instance. We now consider these cases separately.
%    
%    \textbf{Case 1.} Assume that $y_s$ and $y_t$ appear in the 2-SAT instance. In this case there exists a unique maximal path $P$ of $(V,\overline{E}^*)$ (where $\overline{E}^*$ is the set of undirected edges we considered when we constructed the current 2-SAT instance) such that both $s$ and $t$ belong to $P$. Notice that, in Step 2, we have guaranteed that the values $y_s$ and $y_t$ agree (either move only through the path $P$ or we leave the path from one end and enter in the other). Indeed this is forced by the clauses $(y_s \lor \neg y_t)$ and $(\neg y_s \lor y_t)$. Also, in the same step, we have guaranteed that the directions of the edges in $P$, indicated by the edge variables, will agree with the path indicated by the values $y_s$ and $y_t$ (by adding the appropriate path orientation clauses). 
%    
%    Therefore, the only reason that the $s$-$t$ path may not exist in $D$ is if we assume that it moves outside $P$ and there is no path that connects (appropriately) the end points of $P$ in $D$. However, (in the same step) we have added the appropriate directed path clauses so this will never happen. Therefore, the $s$-$t$ path must exist in $D$.
%
%    \textbf{Case 2.} Assume that $x_s$ and $x_t$ appear in the 2-SAT instance. Here we have two paths $P$ and $Q$ of $(V,\overline{E}^*)$ (where $\overline{E}^*$ is the one we considered when we constructed the current 2-SAT instance) such that $s$ belongs to $P$ and $t$ belongs to $Q$. Notice that, we have included path orientation clauses (in Step 2) that guarantee that the orientation indicated by the edge variables allows $s$ to reach one of the end vertices of $P$ (the one indicated by the value of $x_s$). The same is true for $t$. 
%    
%    Therefore, we need to prove that there exists a directed path (using edges of $\hat{A}^*$) that starts from the selected vertex of $P$ and ends at the selected vertex of $Q$. Notice that, this can be guaranteed by the directed path clauses. Indeed if the combination $(x_s,x_t)$ requires the existence of a specific directed path and this path does not exist, we have added appropriate clauses that do not allow the specific combination. Therefore, there exists an $s$-$t$ path in $D$.
%    
%    This completes the correctness of the algorithm and the proof.
%  
%    
%    
%\end{proof}


==> Sections/fpt_tw+k_mso_2-old.tex <==
\section{FPT algorithm by treewidth plus numebr of terminal pairs}

In this section we present an MSO\textsubscript{2} formulation of the Steiner Orientation problem.

Over the years, MSO\textsubscript{2} has been extensively used to model graph problems. The reason is that Courcelle's Theorem states that any graph property expressible in MSO\textsubscript{2} can be decided in FPT time when parameterized by $\tw + |\phi|$, where $\tw$ is the treewidth of the graph and $|\phi|$ is the length of the formula~\cite{Courcelle90}.

The main syntactic elements available in MSO\textsubscript{2} are as follows:
\begin{itemize}
    \item {1. Variables}
    \begin{itemize}
        \item \textbf{First-order variables} (can represent vertices/edges)    
        \item \textbf{Second-order variables} (can represent sets of vertices, edges or arcs)
    \end{itemize}
    \item {2. Set operations}
    \begin{itemize}        
        \item \textbf{Membership} $x \in X $
        \item \textbf{Subset} $X_1\subseteq X_2$
        \item \textbf{Intersection} $X_1 \cap X_2$
        \item \textbf{Union} $X_1 \cup X_2$
    \end{itemize}            
    \item{3. Quantifiers $\forall$ and $\exists$}
    \begin{itemize}
        \item \textbf{First-order quantification}:   
        \begin{align*}
            \forall_{x \in X} \ \phi(x)  & \quad \text{Property over all elements of a set}\\
            \exists_{x \in X} \ \phi(x)  & \quad \text{Existence of an element that satisfies a property}
        \end{align*}
        \item \textbf{Second-order quantification}:
        \begin{align*}
            \forall_{X' \subseteq X}\ \phi(X') & \quad \text{Property over any subset of a set} \\
            \exists_{X' \subseteq X}\ \psi(X') & \quad \text{Existence of a subset that satisfies a property}
        \end{align*}
    \end{itemize}
    
    \item {4. Standard Boolean operators}
    \[
        \land \quad \lor \quad \lnot \quad \Rightarrow \quad \Leftrightarrow
    \]
\end{itemize}
Using the previous we can also define some basic graph notations. In particular, we will use some of the following:
\begin{itemize}
    \item {Basic graph relations}:
        \begin{align*}
            u = v                 & \quad \text{Vertex/edge/arc equality} \\
            \text{edge}(v,u)   & \quad \text{Existence of the edge}  \{v,u\} \\
            \text{arc}(v,u)   & \quad \text{Existence of the arc}  (v,u) \\
            \text{out}(v,a)  & \quad \text{The arc } a \text{ is an outgoing arc of the vertex } v \\
            \text{in}(v,a)  & \quad \text{The arc } a \text{ is an incoming arc of the vertex } v \\
            \text{orientation}(e,a) & \quad \text{The arc } a \text{ is an orientation of the edge } e 
        \end{align*}
\end{itemize}

In our formula, we ask whether there exists an orientation $\lambda$ of the edge set $E$ such that all terminals are connected in $G_\lambda$.

In the first step, we will show how to determine whether a given set of arcs $\vec{E}$ describes a valid orientation of $E$. For each arc $a \in \vec{E}$, we must verify:
\begin{itemize}
    \item There exists an edge $e \in E$ such that $a$ is an orientation of $e$ (checked using $\text{orientation}(e,a)$)
    \item No edge $e \in E$ is oriented in both directions in $\vec{E}$ (i.e., there are no distinct $a_1, a_2 \in \vec{E}$ with $\text{orientation}(e,a_1) \land \text{orientation}(e,a_2)$)
\end{itemize}
In MSO\textsubscript{2} this can be formulated as:

\begin{align*}
    \text{IsOrientation}(\vec{E},E)= & \forall_{a\in \vec{E}}(\exists_{e\in E} \text{orientation}(e,a)) \land \\ & \forall_{a,a' \in \vec{E}} (( \text{orientation}(e,a) \land \text{orientation}(e,a') )\implies a=a')
\end{align*}

In the second step, we give an MSO\textsubscript{2} formula that checks whether a set of directed edges $A'$ contains a directed path between two vertices $v$ and $u$. The formula we create verifies that:
\begin{itemize}
    \item $v$ has exactly one outgoing arc in $A'$ and no incoming arcs,
    \item $u$ has exactly one incoming arc in $A'$ and no outgoing arcs,
    \item Every vertex $w$ incident to arcs in $A'$ (excluding $v$ and $u$) has exactly one incoming and one outgoing arc in $A'$.
\end{itemize}
Note that any set $A'$ that satisfies the previous conditions may not be a simple (directed) path, as it may also contain directed cycles. However, the conditions ensure the existence of a directed $v$-$u$ path using arcs from $A'$. 

We split the formula into four parts. First, we give a formula that checks whether a vertex set $P$ contains exactly those vertices incident to arcs of $A'$, excluding $v$ and $u$.
\begin{align*}
\text{PathVertices}(v,u,P,A')=
& (u \notin P) \land (v \notin P) \land \\ 
& \forall_{w \in P}\exists_{a \in A'}  (\text{out}(w,a) \lor \text{in}(w,a)) \land \\ 
& \forall_{a \in A'}\exists_{w \in P} (\text{out}(w,a) \lor \text{in}(w,a))    
\end{align*}

The second formula verifies that each vertex in $P\setminus\{v,u\}$ has exactly one incoming and one outgoing arc.
\begin{align*}
\text{OneOfEach}(v,u,P,A')= & \text{PathVertices}(v,u,P,A) \land \\ &
\forall_{w\in P} \exists_{a \in A'} \text{in}(w,a) \land \\ &
\forall_{w\in P} \exists_{a \in A'} \text{out}(w,a) \land\\ &
\forall_{a,a'\in A'} ((\exists_{w\in P} \text{in}(w,a) \land \text{in}(w,a')) \implies a=a') \land\\ &
\forall_{a\in A'} ((\exists_{w\in P} \text{out}(w,a) \land \text{out}(w,a')) \implies a=a') 
\end{align*}

Next, we create a formula that checks whether $v$ has exactly one outgoing arc.
\begin{align*}
\text{OutgoingPath}(v,A')= & \exists_{a \in A'} (\text{out}(v,a)) \land \\ 
& \forall_{a,a' \in A'} (\text{out}(v,a) \land \text{out}(v,a) \implies a=a'  ) \land \\ 
&    \forall_{a \in A'} (\neg \text{in}(v,a))\end{align*}

Finally, we check whether $u$ has exactly one incoming arc.
\begin{align*}
\text{IncomingPath}(u,A')= & \exists_{a \in A'} (\text{in}(u,a)) \land \\ 
& \forall_{a,a' \in A'} (\text{in}(u,a) \land \text{in}(u,a) \implies a=a'  ) \land \\ 
&    \forall_{a \in A'} (\neg \text{out}(u,a))
\end{align*}


We combine all the previous formulas to check whether a set of arcs contains a directed $v$-$u$ path as follows:
\begin{align*}
    \text{Path}(v,u,A')= & \exists_{P\subseteq V} (
\text{PathVertices}(v,u,P,A') \land \\ & \text{OneOfEach}(v,u,P,A') \land \\ & \text{OutgoingPath}(v,A') \land \\& \text{IncomingPath}(u,A'))
\end{align*}

Finally,$\SO$ can be expressed in MSO\textsubscript{2} as follows:
\begin{align*}
\SO = \exists_{\vec{E}\subseteq V \times V} \text{IsOrientation}(\vec{E},E) \bigwedge_{i=1}^k (\exists_{A_i\subseteq A\cup\vec{E}} \text{Path}(s_i,t_i,A_i)) 
\end{align*}

Note that our formula has length bounded by a function of $k$, where $k=|\terminals|$. Therefore, using Courcelle's Theorem, we can conclude that $\SO$ is FPT when parameterized by $k + \tw$.


==> Sections/kernel_vc+_T__-old.tex <==

\section{Kernelization}
\begin{theorem} \label{thm:poly:kernel:vc:and:terminals}
Any instance $(G,\terminals)$ of \SO\ admits a kernel of size $\frac{\vc^2}{2}+ \vc + 2k$, where $\vc$ is the size of a minimum vertex cover of $G$ and $k$ is the number of terminal pairs. 
\end{theorem}

\begin{proof}
    \nikos{I will check it again for typos and minor improvements (sorry but it needs a lot of work) - also I will check for inconsistencies like edges $\{\}$ - arcs $()$}
    \nikos{Please do not hesitate to leave comments}

    \textcolor{red}{maybe we can remove the red}
    \textcolor{red}{We assume that the given graph does not have any cycles (directed, undirected, or mixed)\edouard{you can cite \Cref{prop:prepoc}}. Otherwise, we can find such a cycle and contract all its edges and arcs. Also, notice that this does not increase the vertex cover of the graph.}
We begin by computing a minimum vertex cover of the underlying undirected graph of $G$. 
Let $S$ denote this vertex cover, and let $I = V \setminus S$ be the corresponding independent set.  
Define $I_T \subseteq I$ to be the set of vertices that appear in a terminal pair, and let $I_N = I \setminus I_T$ be the remaining vertices of $I$.

If there exists a directed $u$–$v$ path in $G$ for some pair $u, v \in S$, then we explicitly add the arc $(u, v)$ to $A(G)$.  
Note that adding $(u,v)$ is safe, as it does not affect the feasibility of the original instance.
From now on, we assume that $G$ has been modified to include these arcs.

The high-level idea behind the kernel construction is that the vertices in $I_N$ 
will only appear as internal vertices in paths connecting terminals. 
Specifically, they will be used to connect vertices of the vertex cover.  
Our first step is to identify pairs of vertex cover vertices that may require such intermediaries i.e., pairs $(u, v)\in S \times S$ not already directly connected by an arc or edge.

Let $X \subseteq S \times S$ be the set of (ordered) vertex pairs $(u, v)$ with $u \ne v$, such that:
\begin{itemize}
    \item $(u, v) \notin A(G)$, $\{u, v\} \notin E(G)$ and
    \item there exists a path $u - w - v$ in $G$ with $w \in I_N$.
\end{itemize}

Note that $|X| < \vc^2$.  These pairs will help us to select a subset $I' \subseteq I_N$, which we will include in our kernel.

\proofsubparagraph{Creating the kernel:}

Let $|X| = \ell$, and let $(u_j, v_j)$, for $j \in [\ell]$, be an enumeration of the pairs in $X$.

We now construct an undirected auxiliary graph $H = (V', E')$ as follows:
\begin{itemize}
    \item For each pair $(u_j, v_j) \in X$, create a vertex $x_j$.
    \item For each vertex $w \in I_N$, create a vertex $w'$.
    \item We defined $V'$ as $\{x_j \mid (u_j, v_j) \in X\} \cup \{w' \mid w \in I_N\}$.
    \item We add an edge $\{x_j, w'\}$ to $E'$ if one of the following holds:
    \begin{itemize}
        \item $\{u_j, w\}, \{v_j, w\} \in E(G)$,
        \item $\{u_j, w\} \in E(G)$ and $(w, v_j) \in A(G)$,
        \item $(u_j, w) \in A(G)$ and $\{v_j, w\} \in E(G)$.
    \end{itemize}
\end{itemize}

We compute a maximum matching $M \subseteq E'$ in $H$.  
We say that a pair $(u_j, v_j)$ is \textit{matched} to a vertex $w \in I_N$ if $\{x_j, w'\} \in M$.  
Now, we define $I'$ using $M$ as follows; for each such edge $\{x_j, w'\} \in M$, we include the corresponding vertex $w$ in the set $I'$.  

Note that $|I'| < \vc^2$, as we include at most one vertex per pair in $X$ and $|X| < \vc^2$.  
We now strengthen this bound by proving that $|I'| \le \frac{\vc^2}{2}$.

Specifically, we claim that there do not exist two matched edges $\{x_j, w'\}, \{x_{j'}, y'\} \in M$ such that  
$(u_j, v_j) = (u, v)$ and $(u_{j'}, v_{j'}) = (v, u)$.  
Since $M$ is a matching, we know that $w' \ne y'$.  
This would imply that $G$ contains both a path $u - w - v$ and a path $v - y - u$, which together form a cycle.  
This contradicts the assumption that $G$ is acyclic.  
Therefore, such a pair of edges cannot exist in $M$, and thus $|M| \le \binom{\vc}{2} \le \frac{\vc^2}{2}$.  
Hence, $|I'| \le \frac{\vc^2}{2}$.

Having selected $I'$, we have completed the construction of the kernel.  
In particular, we define the kernel to be the subgraph $G[S \cup I_T \cup I']$ along with the terminal pairs $\terminals$. We will denote this subgraph by $G^*$.  

We will show that $(G^*, \terminals)$ is a yes-instance of \SO\ if and only if $(G, \terminals)$ is a yes-instance of \SO.

\proofsubparagraph{Equivalence of the two instances:}

Observe that $G^*$ is an induced subgraph of $G$.  
Therefore, if there exists an orientation $\lambda$ of the edges of $G^*$ such that, for every terminal pair $(s, t) \in \terminals$, there exists a directed $s$–$t$ path in $G^*_\lambda$, then this orientation can be extended to all edges of $G$ by orienting the remaining edges arbitrarily.  
Hence, if $(G^*, \terminals)$ is a yes-instance of \SO, then so is $(G, \terminals)$.
It thus remains to prove the converse direction.

In particular, we need to prove that given an orientation $\lambda$ of $E(G)$ such that, for every $(s,t) \in \terminals$, the graph $G_\lambda$ contains a directed $s$–$t$ path, we can compute an orientation $\mu$ of $E(G^*)$ such that, for every $(s,t) \in \terminals$, the graph $G^*_\mu$ contains a directed $s$–$t$ path.

Assume we are given such an orientation $\lambda$.  
For each $i \in [k]$, let $P_i$ be a shortest directed path from $s_i$ to $t_i$ in $G_\lambda$.

We say that a pair $(u,v) \in S \times S$ \textit{appears} in a path $P$ if there exists a vertex $w \in I_N$ such that the subpath $u - w - v$ is contained in $P$.  
Moreover, if $(u,v)$ appears in $P$, we say that $(u,v)$ \textit{uses} the vertex $w$ in $P$ if $u - w - v$ is a subpath of $P$.

Note that if a pair $(u,v)$ appears in any of the paths $P_i$, for some $i \in [k]$, then $(u,v) \in X$.  
Otherwise, the edge $(u,v)$ would belong to $A(G^*)$ \edouard{ or $E(G^*)$?}, contradicting the assumption that $P_i$ is a shortest path between $s_i$ and $t_i$.

The next step in proving the equivalence of the two instances is to establish the following claim.


\begin{claim} \label{claim:pairs:using:same:vertex}
    If a pair $(u,v) \in S \times S$ appears in any of the paths $P_i$, for $i \in [k]$, then $(u,v)$ can use the same vertex in all its appearances.
\end{claim}
    
\begin{claimproof}
    We proceed by fixing a pair $(u,v) \in S \times S$ that appears in some of the paths $P_i$, for $i \in [k]$.  
    We will modify the paths $P_i$, for $i \in [k]$, so that $(u,v)$ uses the same vertex in every path in which it appears.
    
    Consider a path $P \in \{P_i \mid i \in [k]\}$ such that $(u,v)$ appears in $P$, and let $w$ be the vertex that is used by $(u,v)$ in $P$.  
    We then identify every appearance of $(u,v)$ in all paths $P_i$, for $i \in [k]$, and replace the vertex it uses with $w$.
    
    After this modification, each $P_i$ remains a walk in $G_\lambda$.  
    We now argue that all modified $P_i$ are still paths.\edouard{do we care that they are indeed paths?}  
    Assume, that a $P_i$, for some $i \in [k]$, is no longer a path.  
    This implies that $w$ appears more than once in $P_i$.  
    Therefore, we can obtain a path $Q$ that is strictly shorter than $P_i$ and still connects $s_i$ to $t_i$.  
    This contradicts the assumption that the original $P_i$ was a shortest path.
    
    Finally, we repeat this process until every pair $(u,v)$ that appears in the paths $P_i$, for $i \in [k]$, uses the same vertex in all its appearances.
\end{claimproof}

Hereafter, we assume that the paths $P_i$, for $i \in [k]$, have been selected so that any pair that appears in any of the paths always uses the same vertex.  
Let $X_P$ denote the subset of pairs in $X$ that appear in at least one of the paths $P_i$, for $i \in [k]$.

The next step is to show how the vertices of $I'$ can be used to replace those vertices that are used by the pairs but do not belong to $I'$.

\proofsubparagraph{High-level idea:}

In this part, we sketch the remainder of the proof without providing full details.

The key idea for the construction of $\mu$ and the paths is to partition both $I'$ and the set of terminal pairs $X_P$ into two subsets each:
\begin{itemize}
    \item $I'$ into $I'_1$ and $I'_2$; 
    \item $X_P$ into $X_1$ and $X_2$.
\end{itemize}
These partitions are chosen so that:
\begin{itemize}
    \item Each pair in $X_1$ uses a vertex from $I'_1$ in some path $P_i$, for $i \in [k]$;
    \item Each pair in $X_2$ is matched to a vertex in $I'_2$ by the matching $M$.
\end{itemize}

Now, assuming that $I'_1$ and $I'_2$ are given, we define the orientation $\mu$ of the edges in $E(G^*)$ as follows.  
For each vertex $w \in I'_2$, we orient the edges incident to $w$ so that $(u_j, w) \in A(G^*_\mu)$ and $(w, v_j) \in A(G^*_\mu)$, according to the pair $(u_j, v_j)$ matched to $w$ by $M$.  
If the orientation is not determined by the matching, we choose it arbitrarily.  
All remaining edges are oriented in $\mu$ as in $\lambda$.

Note that, given the above partitioning and the definition of $\mu$, the following holds:
\begin{itemize}
    \item For any pair $(u, v)$ appearing in a path $P_i$ with a subpath $v - w - u$:
    \begin{itemize}
        \item If $(u, v) \in X_1$, then $w \in I'_1$, and the subpath $v - w - u$ is directed in $G^*_\mu$ because $\mu$ and $\lambda$ agree on the orientation of edges incident to $I'_1$;
        \item If $(u, v) \in X_2$, then $(u, v)$ is matched to some $w' \in I'_2$, and this $w'$ can be used to replace $w$ in a directed $u$-$v$ path in $G^*_\mu$ by construction of $\mu$.
    \end{itemize}
\end{itemize}

This implies that the paths $P_i$ can be modified accordingly to form $s$-$t$ paths in $G^*_\mu$.

We now proceed with the details of this construction.

\proofsubparagraph{Partition of $I'$ and $X_P$:}

We begin by defining the set $X^1 \subseteq X_P$ such that a pair $(u_j, v_j) \in X^1$, $j \in [\ell]$, if and only if there is no edge $(x_j, w') \in M$. Observe that any pair in $X^1$ does not use a vertex $v \in I_N \setminus I'$, as in that case $M \cup \{ \{x_j, v'\} \}$ would be a matching in $H$ of size greater than $|M|$, which is a contradiction.

The construction of $I'_1$ proceeds inductively. We start by defining the set $I^1 \subseteq I$ as the set of vertices used by the pairs $(u,v) \in X^1$. Then, let $X^2 \subseteq X_P$ be the set of pairs matched to vertices in $I^1$ by the matching $M$ in $H$. Note that, since $I^1 \cap I_T$ may be nonempty, not all vertices in $I^1$ are necessarily matched to pairs in $X_P$, but this does not affect the construction.
\edouard{I propose to separate the definition of the $X^i,I^i$ and the definition and proof of the invariant} 
Before constructing $I^2$ using $X^2$, we establish a key property: for any pair $(u,v) \in X^2 \setminus X^1$, the vertex used in the paths $P_i$, $i \in [k]$, must belong to $I' \cup I_T$. Suppose, for contradiction, that a pair $(u,v) = (u_j, v_j)$, for some $j \in [\ell]$, uses a vertex $v \in I_N \setminus I'$. Then in $H$ there exists a path $Q$ from $x_j$ to some vertex $x_{j'} \notin V(M)$, where $(u_{j'}, v_{j'}) \in X^1$. This path $Q$ alternates between edges in $M$ and edges in $E(H) \setminus M$. As a result, the set $M \setminus Q \cup (Q \setminus M) \cup \{ \{x_j, v'\} \}$ forms a matching larger than $M$, contradicting its maximality.

Assume we have already constructed the sets $I^q$ and $X^{q+1}$ for some $q \geq 2$, and suppose that for each pair $(u_j, v_j) \in X^{q+1} \setminus X^q$:
\begin{itemize}
    \item The pair uses a vertex $w \in I' \cup I_T$ in every path $P_i$ it appears in, and
    \item There exists a pair $(u_{j'}, v_{j'}) \in X_1$ such that $x_j$ and $x_{j'}$ are connected in $H$ via a path $Q$ alternating between edges in $M$ and $E(H) \setminus M$.
\end{itemize}

We now define $I^{q+1}$ and $X^{q+2}$. The set $I^{q+1}$ is obtained by adding to $I^q$ all vertices used by the pairs in $X^{q+1} \setminus X^q$. Since these vertices are used in paths and come from $X^{q+1}$, we know $I^{q+1} \subseteq I' \cup I_T$. Then we define $X^{q+2}$ as the union of $X^{q+1}$ and all pairs in $X_P$ that are matched to vertices in $I^{q+1} \setminus I^q$.

We now prove that $X^{q+2}$ satisfies the same properties as $X^{q+1}$.

First, consider any pair $(u_j, v_j) \in X^{q+2} \setminus X^{q+1}$. We will show that there exists a pair $(u_{j'}, v_{j'}) \in X_1$ and an alternating path in $H$ between $x_j$ and $x_{j'}$. Assume otherwise. Let $w \notin I' \cup I_T$ be the vertex used by $(u_j, v_j)$. Since $(u_j, v_j) \in X^{q+2} \setminus X^{q+1}$, it is matched to some vertex $v \in I^{q+1}$, and there exists a pair $(u_{j''}, v_{j''}) \in X^{q+1} \setminus X^q$ such that:
\begin{itemize}
    \item $(x_j, v') \in M$ (because $(u_j, v_j)$ is in $X^{q+2} \setminus X^{q+1}$), and
    \item $(x_{j''}, v') \in E(H)$ (since the pair $(u_{j''}, v_{j''})$ must use $v'$ and hence $v \in I^{q+1}$).
\end{itemize}
By the inductive assumption, there exists a path $Q$ in $H$ between $x_{j''}$ and $x_{j'}$, for some $(u_{j'}, v_{j'}) \in X_1$, alternating between edges in $M$ and $E(H) \setminus M$. Since $H$ is bipartite and $x_{j''}$ is an endpoint of $Q$, the edge incident to $x_{j''}$ in $Q$ belongs to $M$. Therefore, we can extend $Q$ to a path from $x_j$ to $x_{j'}$ by adding the edges $\{x_j, v'\} \in M$ and $\{x_{j''}, v'\} \in E(H)$, preserving the alternating property.

Next, we show that every pair $(u_j, v_j) \in X^{q+2} \setminus X^{q+1}$ uses a vertex $w \in I' \cup I_T$ in all paths $P_i$ it appears in. Suppose this is false and $w \in I_N \setminus I'$. Then, using the constructed alternating path $Q$ from the previous argument, the set $(M \setminus Q) \cup (Q \setminus M) \cup \{x_j, w'\}$ would be a matching in $H$ of size $|M| + 1$, again a contradiction.

We terminate the construction when $I^{q+1} \setminus I^q = \emptyset$. We then define $I'_1 = I^{q+1}$ and $I'_2 = I' \setminus I'_1$. Finally, we define a partition of $X_P$ as follows: let $X_{I_T}$ be the set of pairs $(u,v) \in X_P$ such that the vertex used by $(u,v)$ lies in $I_T$. Then, set $X_1 = X_{I_T} \cup X^{q+2}$ and $X_2 = X_P \setminus X_1$.


\proofsubparagraph{Properties of $X_2$ and construction of the new paths:}

Before proceeding, observe that any pair $(u,v) \in X_2$ has been matched by $M$ to a vertex $w \in I'_2$.  
Indeed, if $(u,v)$ had not been matched to a vertex in $I'_2$, then either it was not matched at all, or it was matched to a vertex in $I'_1$.  
In the first case, we would have $(u,v) \in X^1 \subseteq X_1$, contradicting $(u,v) \in X_2$.  
In the second case, the matched vertex belongs to $I^{q+1}$, implying $(u,v) \in X^{q+2} \subseteq X_1$, again a contradiction.

Next, recall the definition of $\mu$.  
For every vertex $w \in I'_1 \cup I_T$, the orientation $\mu$ agrees with $\lambda$ on the edges incident to $w$.  
Then, for each vertex $w \in I'_2$ matched by $M$ to some pair $(u,v)$, we set $\mu$ to orient the edges incident to $w$ so that $(u,w)$ and $(w,v)$ are arcs in $A(G^*_\mu)$.  
This orientation is valid due to the construction of the graph $H$ and the properties of the matching $M$.

We now claim that for all $i \in [k]$, the graph $G^*_\mu$ contains a directed $s_i$-$t_i$ path.  
To prove this, we modify the paths $P_i$ accordingly.  
Our goal is to ensure that every pair $(u,v) \in X$ appearing in the paths $P_i$ uses only vertices from $I'$, and moreover, that $\mu$ orients the relevant edges to allow such usage in $G^*_\mu$.

Fix a pair $(u,v)$ that appears in some $P_i$.  
If $(u,v) \notin X_2$, then it uses a vertex $w \in I'_1 \cup I_T \subseteq V(G^*_\mu)$.  
Since $\mu$ agrees with $\lambda$ on edges incident to these vertices, we conclude that the arcs $(u,w)$ and $(w,v)$ are present in $A(G^*_\mu)$.

Now consider the case where $(u,v) \in X_2$, and let $w$ be the vertex it uses in the paths.  
Since $(u,v)$ has been matched to a vertex $z \in I'_2$ by $M$, and $\mu$ orients the edges so that $(u,z)$ and $(z,v)$ are arcs in $G^*_\mu$, we can modify every path where $(u,v)$ uses $w$ by replacing $w$ with $z$.  
We apply this modification for all such pairs in $X_2$.

After these modifications, each $P_i$ becomes a walk in $G^*_\mu$ (since vertices may be repeated), but this suffices to guarantee the existence of $s_i$-$t_i$ paths for all $i \in [k]$.

This shows that if $(G, \terminals)$ is a yes-instance of \SO, then so is $(G^*, \terminals)$.

Finally, recall the bound on the kernel size.  
We have $G^* = G[S \cup I' \cup I_T]$.  
Since $|I'| \le \frac{\vc^2}{2}$ and $|I_T| \le 2|\terminals| = 2k$, the total size of $S \cup I_T \cup I'$ is at most $\vc + 2k + \frac{\vc^2}{2}$.  
Therefore, $G^*$ together with $\terminals$ forms a kernel of size at most $\vc + 2k + \frac{\vc^2}{2}$.

\end{proof}

    %%%%%%%%%%%%%%%%%
\begin{theorem}
    Any instance $(G,\terminals)$ of \SO, where no vertex of $V(G)$ appears in more than one terminal pair, admits a kernel of size $O(2^{\vc})$, where $\vc$ is the size of a minimum vertex cover of $G$. 
\end{theorem}

\begin{proof}We start by assuming that the given instance $(G,\terminals)$ is the kernel obtained by Theorem~\ref{thm:poly:kernel:vc:and:terminals}.
Let $S$ be a minimum vertex cover of $G$, $I = V(G) \setminus S$ a maximum independent set, $I_T \subseteq I$ the subset of vertices in the independent set that appear in terminal pairs, and $I' = V(G) \setminus (S \cup I_T)$.
From the size bound of the kernel, we have $|I'| \le \frac{\vc^2}{2}$, where $\vc = |S|$.

The high-level idea is to classify terminal pairs based on the neighborhoods (both in $E$ and $A$) of their source and sink terminals.
For each type, we keep four representative terminal pairs and we remove the rest. Then we delete any vertex of $I_T$ that no longer appears in a terminal pair.
Finally, we will show that this new instance is equivalent to $(G,\terminals)$ and that its size is bounded by $2^{O(\vc)}$.

\proofsubparagraph{Types of terminals}

We consider terminal pairs $(s,t) \in \terminals$ with $s,t \in I_T$.
First, we define types of vertices in $I_T$: two vertices in $I_T$ are of the same type if they have identical neighborhoods in both $E$ and $A$.
Next, we refine each vertex type into two subtypes, one containing all source terminals and one containing all sink terminals of the original type.
Since $G$ is a mixed graph, this yields $4^{\vc}$ types of source terminals and $4^{\vc}$ types of sink terminals.
We then add $\vc$ types, each corresponding to a vertex in $S$ (recall that $S$ is a vertex cover of $G$).
Because every terminal lies in $I_T \cup S$, we define types of terminal pairs using the $2 \cdot 4^{\vc} + \vc$ types constructed.

Specifically, two terminal pairs $(s,t)$ and $(s',t')$ are of the same type if $s$ and $s'$ share the same type and $t$ and $t'$ share the same type.
Note that the total number of terminal pair types is $2^{O(\vc)}$.

\proofsubparagraph{Creating the kernel}

Now, for each type of terminal pairs, if the number of terminal pairs of this type is at most $4$, we keep all such pairs and the vertices appearing in them. Otherwise, we arbitrarily select four terminal pairs of that type and remove all other terminal pairs of that type from $\terminals$.  
Let $\terminals^*$ be the resulting set of terminal pairs. Finally, we delete any vertex $v \in I_T$ that does not appear in any terminal pair of $\terminals^*$.  

Let $(G^*, \terminals^*)$ be the resulting instance. Notice that $V(G^*) = S \cup I' \cup I_T'$, where $I_T' \subseteq I_T$ and $|I_T'| \leq 2|\terminals^*|$. Since we have kept $2^{O(\vc)}$ terminal pairs and $|S \cup I'| \leq \vc + \binom{\vc}{2}$, we conclude that $|V(G^*)| = 2^{O(\vc)}$.

It remains to show that $(G^*, \terminals^*)$ is equivalent to $(G, \terminals)$.


\proofsubparagraph{Equivalence of the two instances}

For the first direction, assume that $(G^*, \terminals^*)$ is a yes-instance and let $\lambda$ be an orientation of $E(G^*)$ such that, for every terminal pair $(s,t) \in \terminals^*$, there exists a directed $s$-$t$ path in $G^*_\lambda$.  
We construct an orientation $\mu$ of $E(G)$ as follows:
\begin{itemize}
    \item $\mu$ agrees with $\lambda$ on every edge in $E(G) \cap E(G^*)$.  
    \item For every edge $e \in E(G) \setminus E(G^*)$:
    \begin{itemize}
        \item Let $v \in I_T \setminus I_T'$ be the vertex incident to $e$ (such $v$ must exist by the construction of $G^*$).
        \item Let $(s,t) \in \terminals$ be the terminal pair containing $v$.  
        \item Select arbitrarily a pair $(s', t') \in \terminals^*$ such that $(s,t)$ and $(s', t')$ are of the same type.
        \item Let $v' \in \{s', t'\}$ be the terminal with the same type as $v$.
        \item Orient the edges incident to $v$ in $\mu$ the same way as $\lambda$ orients the edges incident to $v'$.
    \end{itemize}
\end{itemize}

Note that, since terminals do not overlap, the orientation $\mu$ is well defined.  
We now prove the following claim:
\begin{claim}
    For all pairs $(s,t)\in \terminals$ there exists a directed $s$-$t$ path in $G_{\mu}$. 
\end{claim}

\begin{claimproof}
    Since $\mu$ extends $\lambda$ and $G^*$ is an induced subgraph of $G$, any directed path in $G^*_{\lambda}$ is also a directed path in $G_{\mu}$.
    Therefore, for any $(s',t')\in \terminals \cap \terminals^*$, there exists a directed $s'$-$t'$ path in $G_{\mu}$.

    Now consider a pair $(s,t) \in \terminals \setminus \terminals^*$. By the construction of $\terminals^*$, there exists a pair $(s',t')\in \terminals^*$ such that $(s,t)$ and $(s',t')$ have the same terminal type.
    We will prove that there exists a directed $s$-$t$ path $P$ in $G_{\mu}$ using the $s'$-$t'$ path $P'$.

    Since $(s,t)$ and $(s',t')$ are of the same terminal type, and terminals do not overlap, we have $s,t,s',t' \in I_T$. Let $s' \rightarrow v_1 \rightarrow \ldots \rightarrow v_2 \rightarrow t'$ be the path $P'$ (where $v_1$ and $v_2$ may coincide).
    
    By construction, $\mu$ orients the edges incident to $s$ in the same way as those incident to $s'$. Since $(s',v_1)\in A(G_{\mu})$, it follows that $(s,v_1)\in A(G_{\mu})$. Similarly, since $(v_2,t')\in A(G_{\mu})$, we have $(v_2,t)\in A(G_{\mu})$.

    Therefore, we obtain a directed $s$-$t$ path in $G_{\mu}$.
\end{claimproof}

Due to the previous claim, we conclude that if $(G^*,\terminals^*)$ is a yes-instance, then $(G,\terminals)$ is also a yes-instance. It remains to prove the converse.

Assume that $(G,\terminals)$ is a yes-instance and let $\lambda$ be an orientation such that, for each $(s_i,t_i)\in \terminals$, there exists a directed path $P_i$ in $G_{\lambda}$. 
Before we define the orientation $\mu$ for the edges in $E(G^*)$, we will modify the paths $P_1,\ldots,P_k$ so that they satisfy certain structural properties.

The next claim is crucial for the correctness of this theorem.

\begin{claim} \label{claim:two:appearances:of:terminals}
    There exists a set of directed paths $Q_i$, $i \in [k]$, in $G_\lambda$ such that, for each terminal type, at most two source terminals and at most two sink terminals appear in more than one path.
\end{claim}

Before proceeding with the proof of the claim, let us explain its implications.
Observe that the source and sink of each terminal pair must appear at least once, in the path that connects them. All other occurrences of these vertices correspond to intermediate appearances in the paths that connect other terminal pairs.

Since the number of terminal types is bounded by a function of the vertex cover number $\vc$, if the above claim holds, we obtain a small subgraph (of size bounded by a function of $\vc$) that contains all such intermediate vertices of the paths $P_i$, $i \in [k]$.
Therefore, the feasibility of the instance $(G,\terminals)$ depends only on this part of the graph (along with $I'$).

We now proceed with the proof of the claim.
\begin{claimproof}
    It suffices to prove the claim for terminal pair types that do not include vertices from $S$. Indeed, since we have no overlapping terminals, if a type includes a vertex from $S$, it must correspond to exactly one terminal pair. Therefore, the claim trivially holds in such cases.

    Fix a type of terminal pairs, denoted by $p$. Let $\terminals_p$ be the set of all terminal pairs of type $p$, and let $S_p$ and $T_p$ denote the sets of source and sink terminals, respectively, that appear in $\terminals_p$.

    If $|\terminals_p| = 1$, the claim holds trivially. Thus, we assume that $|\terminals_p| \ge 2$. Additionally we can assume that any vertex in $S_p$ is incident to at most one edge in $E(G)$. Indeed,     
    if any vertex in $S_p$ is incident to at least two edges in $E(G)$, 
    then $G$ contains a cycle, contradicting the assumption that $G$ is acyclic. Therefore, for each $s \in S_p$, at most one edge of $E(G)$ is incident to $s$. The same argument holds for each $t \in T_p$.

    Consider a terminal pair $(s,t) \in \terminals_p$. If neither $s$ nor $t$ is incident to any edge in $E(G)$, then the same holds for all other terminal pairs in $\terminals_p$. Furthermore, if any source $s' \in S_p$ is used as an intermediate vertex in some path $P_i$, it can be replaced by $s$ since they share the same incident arcs, regardless of the orientation $\lambda$. The same holds for the sink terminals.

    We now assume that there exists at least one edge in $E(G)$ incident to either $s$ or $t$. Without loss of generality, assume that $s$ is incident to such an edge and let $e_s$ denote this edge. If $e_s = \{s,v\}$ for some $v \in S$, then for all $s' \in S_p$ we have $e_{s'} = \{s',v\} \in E(G)$. Our goal is to modify the set of paths $\{P_i \mid i \in [k]\}$ so that at most two vertices from $S_p$ appear in these paths as intermediate vertices.

    Define the sets $\mathcal{P}^{\mathrm{in}}_p$ and $\mathcal{P}^{\mathrm{out}}_p \subseteq \{P_i \mid i \in [k]\}$ as follows:
    \begin{itemize}
        \item $P \in \mathcal{P}^{\mathrm{in}}_p$ if there exists $(s,t) \in \terminals_p$ such that:
        \begin{itemize}
            \item $P$ is not an $s$-$t$ path,
            \item $e_s = \{s,v\}$, and
            \item $(v,s) \in A(P)$.
        \end{itemize}
        \item $P \in \mathcal{P}^{\mathrm{out}}_p$ if there exists $(s,t) \in \terminals_p$ such that:
        \begin{itemize}
            \item $P$ is not an $s$-$t$ path,
            \item $e_s = \{s,v\}$, and
            \item $(s,v) \in A(P)$.
        \end{itemize}
    \end{itemize}

    Note that $\mathcal{P}^{\mathrm{in}}_p \cup \mathcal{P}^{\mathrm{out}}_p$ contains all paths that use vertices of $S_p$ as intermediate vertices.

    Assume that $\mathcal{P}^{\mathrm{in}}_p$ is non-empty. Arbitrarily select a vertex $s_{\mathrm{in}}$ such that $(v, s_{\mathrm{in}}) \in A(G_\lambda)$. Such a vertex must exist; otherwise, $\mathcal{P}^{\mathrm{in}}_p$ would be empty. In each path $P \in \mathcal{P}^{\mathrm{in}}_p$, if there exists a vertex $s' \neq s_{\mathrm{in}}$ in $S_p$ such that $(u, s'), (s', v) \in E(P)$, we replace these with the edges $(u, s_{\mathrm{in}}), (s_{\mathrm{in}}, v)$. Since $s_{\mathrm{in}}$ and $s'$ are of the same type and $e_{s_{\mathrm{in}}} = \{s_{\mathrm{in}}, v\}$, the edge $(u, s_{\mathrm{in}})$ is valid, and this substitution is always possible.

    We perform an analogous modification for $\mathcal{P}^{\mathrm{out}}_p$. Assuming $\mathcal{P}^{\mathrm{out}}_p$ is non-empty, we select (arbitrarily) a vertex $s_{\mathrm{out}}$ such that $(s_{\mathrm{out}}, v) \in A(G_\lambda)$. In each path $P \in \mathcal{P}^{\mathrm{out}}_p$, if there exists $s' \neq s_{\mathrm{out}}$ in $S_p$ such that $(v, s'), (s', u) \in E(P)$, we replace them with $(v, s_{\mathrm{out}}), (s_{\mathrm{out}}, u)$.

    Note that these modifications may produce walks rather than simple paths. However, since the original paths were shortest paths between terminal pairs, and we preserved their lengths, the resulting walks are also simple paths.

    After these modifications, at most two vertices from $S_p$ ($s_{\mathrm{in}}$ and $s_{\mathrm{out}}$) appear in any path $P_i$ as intermediate vertices. We can apply the same process to ensure that at most two vertices from $T_p$ ($t_{\mathrm{in}}$ and $t_{\mathrm{out}}$) appear in any path as intermediate sink vertices.

    This transformation does not affect the intermediate appearances of terminals from other types. Therefore, applying this process for every terminal type proves the claim.
\end{claimproof}

\proofsubparagraph{Constructing the orientation in $G^*$}

Hereafter, we assume that the given set of paths $\{P_i \mid i \in [k]\}$ satisfies the property of Claim~\ref{claim:two:appearances:of:terminals}.

To define the orientation $\mu$ of the edges in $E(G^*)$, we use terminal pairs whose endpoints appear as intermediate vertices in the paths $\{P_i \mid i \in [k]\}$. Specifically, for each type $p$ of terminal pairs, we select four pairs $(s_p^1, t_p^1), (s_p^2, t_p^2), (s_p^3, t_p^3), (s_p^4, t_p^4) \in \terminals_p$ as follows:
\begin{itemize}
    \item Select all source terminals in $S_p$ that appear as intermediate vertices in any path $P \in \{P_i \mid i \in [k]\}$.
    \item Select all sink terminals in $T_p$ that appear as intermediate vertices in any path $P \in \{P_i \mid i \in [k]\}$.
    \item Let $\terminals_p^{\mathrm{good}}$ be the set of all terminal pairs in $\terminals_p$ that involve the selected source and sink terminals.
\end{itemize}
By Claim~\ref{claim:two:appearances:of:terminals}, we know that there are at most four such terminal pairs. If $|\terminals_p^{\mathrm{good}}| < 4$, we arbitrarily add more terminal pairs from $\terminals_p$ until $|\terminals_p^{\mathrm{good}}| = \min\{4, |\terminals_p|\}$.

Let $\terminals^{\mathrm{good}} = \bigcup_p \terminals_p^{\mathrm{good}}$ be the union over all types $p$.

Recall that, in $G^*$, for each type $p$, we have kept $\min\{4, |\terminals_p|\}$ terminal pairs of type $p$. We arbitrarily define a matching between $\terminals_p^{\mathrm{good}}$ and $\terminals^* \cap \terminals_p$ for each type $p$. Let $m: \terminals^{\mathrm{good}} \rightarrow \terminals^*$ denote this matching.

Let $I_T^{\mathrm{good}}$ be the set of vertices appearing in terminal pairs of $\terminals^{\mathrm{good}}$. Define a matching $N: I_T^{\mathrm{good}} \rightarrow I_T'$ induced by $m$, respecting the role of vertices as sources or sinks; that is, for $m((s, t)) = (s', t')$, we set $N(s) = s'$ and $N(t) = t'$.

We extend $N$ to the entire vertex set $I_T^{\mathrm{good}} \cup S \cup I'$ by setting $N(v) = v$ for all $v \in S \cup I'$. Observe that $N$ now maps $I_T^{\mathrm{good}} \cup S \cup I'$ into $V(G^*) = I_T' \cup S \cup I'$.

We are now ready to define the orientation $\mu$ of the edges in $E(G^*)$: for each edge $\{u, v\} \in E(G^*)$, we orient it in the same direction as $\lambda$ orients the edge $\{N(u), N(v)\} \in E(G)$.

It remains to show that, for every terminal pair $(s, t) \in \terminals^*$, there exists a directed $s$-$t$ path in $G^*_{\mu}$. For this, observe the following:
\begin{itemize}
    \item Any $u$-$v$ path in $G_{\lambda}[I_T^{\mathrm{good}} \cup S \cup I']$ maps to an $N(u)$-$N(v)$ path in $G^*_{\mu}$.
    \item For every $(s, t) \in \terminals^*$, there exists a terminal pair $(s', t') \in \terminals^{\mathrm{good}}$ such that $N(s') = s$ and $N(t') = t$.
    \item Each $(s', t') \in \terminals^{\mathrm{good}}$ is connected via a path $P \in \{P_i \mid i \in [k]\}$ using only vertices in $I_T^{\mathrm{good}} \cup S \cup I'$ as intermediate nodes. Hence, there exists a directed $s'$-$t'$ path in $G_{\lambda}[I_T^{\mathrm{good}} \cup S \cup I']$.
\end{itemize}

Therefore, we conclude that if $(G, \terminals)$ is a yes-instance, then so is $(G^*, \terminals^*)$.

This completes the proof.

\end{proof}
